Electroweak superpartner production at 13.6 TeV with Resummino

Due to the greater experimental precision expected from the currently ongoing LHC Run 3, equally accurate theoretical predictions are essential. We update the documentation of the Resummino package, a program dedicated to precision cross section calculations for the production of a pair of sleptons, electroweakinos, and leptons in the presence of extra gauge bosons, and for the production of an associated electroweakino-squark or electroweakino-gluino pair. We detail different additions that have been released since the initial version of the program a decade ago, and then use the code to investigate the impact of threshold resummation corrections at the next-to-next-to-leading-logarithmic accuracy. As an illustration of the code we consider the production of pairs of electroweakinos and sleptons at the LHC for centre-of-mass energies ranging up to 13.6 TeV and in simplified model scenarios. We find slightly increased total cross section values, accompanied by a significant decrease of the associated theoretical uncertainties. Furthermore, we explore the dependence of the results on the squark masses.

==> tab_higgsino_split_13000.tex <==
$80$ 	&$81.5$ 	&$80.75$ 	&$7765^{+2.5\%+2.8\%}_{-3.6\%-2.8\%}$ 	&$5088^{+2.7\%+2.7\%}_{-3.7\%-2.7\%}$ 	&$6761^{+2.6\%+2.4\%}_{-3.7\%-2.4\%}$ 	&$8113^{+2.6\%+2.7\%}_{-3.8\%-2.7\%}$ 	\\
	 $80$ 	&	 $90$ 	&	 $85$ 	&	 $5837^{+2.3\%+2.8\%}_{-3.3\%-2.8\%}$ 	&	 $3776^{+2.4\%+2.8\%}_{-3.4\%-2.8\%}$ 	&	 $5602^{+2.4\%+2.4\%}_{-3.5\%-2.4\%}$ 	&	 $6544^{+2.5\%+2.7\%}_{-3.6\%-2.7\%}$ 	\\
	 $100$ 	&	 $101.5$ 	&	 $100.8$ 	&	 $3438^{+2.0\%+3.0\%}_{-2.8\%-3.0\%}$ 	&	 $2168^{+2.1\%+2.9\%}_{-2.9\%-2.9\%}$ 	&	 $3043^{+2.1\%+2.6\%}_{-2.8\%-2.6\%}$ 	&	 $3349^{+2.1\%+2.8\%}_{-2.9\%-2.8\%}$ 	\\
	 $100$ 	&	 $110$ 	&	 $105$ 	&	 $2757^{+1.9\%+3.0\%}_{-2.5\%-3.0\%}$ 	&	 $1720^{+2.0\%+3.0\%}_{-2.7\%-3.0\%}$ 	&	 $2628^{+2.0\%+2.6\%}_{-2.7\%-2.6\%}$ 	&	 $2852^{+2.0\%+2.8\%}_{-2.8\%-2.8\%}$ 	\\
	 $60$ 	&	 $120$ 	&	 $90$ 	&	 $2950^{+1.9\%+3.0\%}_{-2.6\%-3.0\%}$ 	&	 $1848^{+2.0\%+2.9\%}_{-2.8\%-2.9\%}$ 	&	 $4555^{+2.3\%+2.5\%}_{-3.3\%-2.5\%}$ 	&	 $4714^{+2.3\%+2.7\%}_{-3.3\%-2.7\%}$ 	\\
	 $125$ 	&	 $128$ 	&	 $126.5$ 	&	 $1512^{+1.5\%+3.2\%}_{-2.1\%-3.2\%}$ 	&	 $913.3^{+1.7\%+3.1\%}_{-2.2\%-3.1\%}$ 	&	 $1360^{+1.6\%+2.8\%}_{-2.1\%-2.8\%}$ 	&	 $1414^{+1.7\%+2.9\%}_{-2.2\%-2.9\%}$ 	\\
	 $100$ 	&	 $140$ 	&	 $120$ 	&	 $1395^{+1.5\%+3.2\%}_{-2.0\%-3.2\%}$ 	&	 $838.8^{+1.7\%+3.2\%}_{-2.1\%-3.2\%}$ 	&	 $1639^{+1.8\%+2.7\%}_{-2.3\%-2.7\%}$ 	&	 $1682^{+1.8\%+2.9\%}_{-2.3\%-2.9\%}$ 	\\
	 $150$ 	&	 $152$ 	&	 $151$ 	&	 $815.4^{+1.3\%+3.4\%}_{-1.6\%-3.4\%}$ 	&	 $474.6^{+1.5\%+3.4\%}_{-1.7\%-3.4\%}$ 	&	 $725^{+1.4\%+2.9\%}_{-1.7\%-2.9\%}$ 	&	 $731.7^{+1.4\%+3.1\%}_{-1.7\%-3.1\%}$ 	\\
	 $100$ 	&	 $160$ 	&	 $130$ 	&	 $943.9^{+1.3\%+3.3\%}_{-1.7\%-3.3\%}$ 	&	 $554.6^{+1.5\%+3.3\%}_{-1.8\%-3.3\%}$ 	&	 $1234^{+1.6\%+2.8\%}_{-2.1\%-2.8\%}$ 	&	 $1219^{+1.6\%+3.0\%}_{-2.1\%-3.0\%}$ 	\\
	 $150$ 	&	 $170$ 	&	 $160$ 	&	 $601.8^{+1.2\%+3.5\%}_{-1.5\%-3.5\%}$ 	&	 $343.7^{+1.3\%+3.5\%}_{-1.6\%-3.5\%}$ 	&	 $589.3^{+1.3\%+3.0\%}_{-1.6\%-3.0\%}$ 	&	 $588^{+1.3\%+3.1\%}_{-1.6\%-3.1\%}$ 	\\
	 $125$ 	&	 $185$ 	&	 $155$ 	&	 $537.9^{+1.1\%+3.6\%}_{-1.4\%-3.6\%}$ 	&	 $305.1^{+1.3\%+3.6\%}_{-1.5\%-3.6\%}$ 	&	 $660.3^{+1.3\%+3.0\%}_{-1.7\%-3.0\%}$ 	&	 $642.5^{+1.4\%+3.1\%}_{-1.7\%-3.1\%}$ 	\\
	 $175$ 	&	 $195$ 	&	 $185$ 	&	 $363.5^{+1.0\%+3.8\%}_{-1.2\%-3.8\%}$ 	&	 $200.8^{+1.2\%+3.8\%}_{-1.3\%-3.8\%}$ 	&	 $348.7^{+1.1\%+3.2\%}_{-1.3\%-3.2\%}$ 	&	 $342.2^{+1.1\%+3.3\%}_{-1.4\%-3.3\%}$ 	\\
	 $150$ 	&	 $210$ 	&	 $180$ 	&	 $329.6^{+1.0\%+3.8\%}_{-1.2\%-3.8\%}$ 	&	 $180.9^{+1.2\%+3.9\%}_{-1.3\%-3.9\%}$ 	&	 $385.2^{+1.1\%+3.1\%}_{-1.4\%-3.1\%}$ 	&	 $371^{+1.2\%+3.3\%}_{-1.4\%-3.3\%}$ 	\\
	 $200$ 	&	 $230$ 	&	 $215$ 	&	 $205.1^{+0.8\%+4.0\%}_{-1.0\%-4.0\%}$ 	&	 $108.9^{+1.0\%+4.2\%}_{-1.1\%-4.2\%}$ 	&	 $200.6^{+1.0\%+3.4\%}_{-1.1\%-3.4\%}$ 	&	 $193.7^{+1.0\%+3.5\%}_{-1.1\%-3.5\%}$ 	\\
	 $225$ 	&	 $240$ 	&	 $232.5$ 	&	 $164.8^{+0.8\%+4.2\%}_{-0.9\%-4.2\%}$ 	&	 $86.07^{+1.0\%+4.3\%}_{-1.0\%-4.3\%}$ 	&	 $149.7^{+0.9\%+3.5\%}_{-1.0\%-3.5\%}$ 	&	 $144.1^{+0.9\%+3.7\%}_{-1.0\%-3.7\%}$ 	\\
	 $200$ 	&	 $260$ 	&	 $230$ 	&	 $143.6^{+0.8\%+4.2\%}_{-0.9\%-4.2\%}$ 	&	 $74.28^{+0.9\%+4.4\%}_{-1.0\%-4.4\%}$ 	&	 $155.9^{+0.9\%+3.5\%}_{-1.0\%-3.5\%}$ 	&	 $148.1^{+0.9\%+3.6\%}_{-1.0\%-3.6\%}$ 	\\
	 $250$ 	&	 $280$ 	&	 $265$ 	&	 $96.84^{+0.7\%+4.5\%}_{-0.7\%-4.5\%}$ 	&	 $48.61^{+0.8\%+4.8\%}_{-0.9\%-4.8\%}$ 	&	 $91.02^{+0.8\%+3.8\%}_{-0.8\%-3.8\%}$ 	&	 $86.63^{+0.8\%+3.9\%}_{-0.8\%-3.9\%}$ 	\\
	 $300$ 	&	 $305$ 	&	 $302.5$ 	&	 $64.16^{+0.6\%+4.8\%}_{-0.6\%-4.8\%}$ 	&	 $31.18^{+0.8\%+5.1\%}_{-0.7\%-5.1\%}$ 	&	 $54.36^{+0.7\%+4.1\%}_{-0.7\%-4.1\%}$ 	&	 $51.45^{+0.7\%+4.2\%}_{-0.7\%-4.2\%}$ 	\\
	 $300$ 	&	 $320$ 	&	 $310$ 	&	 $55.77^{+0.6\%+4.9\%}_{-0.6\%-4.9\%}$ 	&	 $26.8^{+0.7\%+5.3\%}_{-0.7\%-5.3\%}$ 	&	 $49.34^{+0.6\%+4.1\%}_{-0.7\%-4.1\%}$ 	&	 $46.6^{+0.6\%+4.3\%}_{-0.7\%-4.3\%}$ 	\\


==> tab_higgsino_split_13600.tex <==
$80$ 	&$81.5$ 	&$80.75$ 	&$8187^{+2.6\%+2.7\%}_{-3.7\%-2.7\%}$ 	&$5402^{+2.7\%+2.7\%}_{-3.8\%-2.7\%}$ 	&$7152^{+2.6\%+2.4\%}_{-3.8\%-2.4\%}$ 	&$8587^{+2.7\%+2.6\%}_{-3.9\%-2.6\%}$ 	\\
	 $80$ 	&	 $90$ 	&	 $85$ 	&	 $6160^{+2.4\%+2.8\%}_{-3.4\%-2.8\%}$ 	&	 $4014^{+2.5\%+2.7\%}_{-3.5\%-2.7\%}$ 	&	 $5930^{+2.5\%+2.4\%}_{-3.6\%-2.4\%}$ 	&	 $6932^{+2.6\%+2.7\%}_{-3.7\%-2.7\%}$ 	\\
	 $100$ 	&	 $101.5$ 	&	 $100.8$ 	&	 $3635^{+2.0\%+2.9\%}_{-2.9\%-2.9\%}$ 	&	 $2310^{+2.2\%+2.8\%}_{-3.0\%-2.8\%}$ 	&	 $3229^{+2.1\%+2.5\%}_{-3.0\%-2.5\%}$ 	&	 $3556^{+2.2\%+2.7\%}_{-3.0\%-2.7\%}$ 	\\
	 $100$ 	&	 $110$ 	&	 $105$ 	&	 $2918^{+1.9\%+3.0\%}_{-2.6\%-3.0\%}$ 	&	 $1834^{+2.0\%+2.9\%}_{-2.8\%-2.9\%}$ 	&	 $2789^{+2.0\%+2.6\%}_{-2.8\%-2.6\%}$ 	&	 $3030^{+2.1\%+2.8\%}_{-2.9\%-2.8\%}$ 	\\
	 $60$ 	&	 $120$ 	&	 $90$ 	&	 $3121^{+1.9\%+3.0\%}_{-2.7\%-3.0\%}$ 	&	 $1970^{+2.1\%+2.9\%}_{-2.8\%-2.9\%}$ 	&	 $4825^{+2.4\%+2.4\%}_{-3.4\%-2.4\%}$ 	&	 $4998^{+2.4\%+2.7\%}_{-3.4\%-2.7\%}$ 	\\
	 $125$ 	&	 $128$ 	&	 $126.5$ 	&	 $1604^{+1.6\%+3.1\%}_{-2.1\%-3.1\%}$ 	&	 $977.2^{+1.8\%+3.1\%}_{-2.3\%-3.1\%}$ 	&	 $1448^{+1.7\%+2.7\%}_{-2.2\%-2.7\%}$ 	&	 $1507^{+1.7\%+2.9\%}_{-2.3\%-2.9\%}$ 	\\
	 $100$ 	&	 $140$ 	&	 $120$ 	&	 $1480^{+1.6\%+3.2\%}_{-2.1\%-3.2\%}$ 	&	 $897.7^{+1.7\%+3.1\%}_{-2.2\%-3.1\%}$ 	&	 $1743^{+1.8\%+2.7\%}_{-2.4\%-2.7\%}$ 	&	 $1791^{+1.8\%+2.8\%}_{-2.4\%-2.8\%}$ 	\\
	 $150$ 	&	 $152$ 	&	 $151$ 	&	 $867^{+1.3\%+3.3\%}_{-1.7\%-3.3\%}$ 	&	 $509.6^{+1.5\%+3.3\%}_{-1.8\%-3.3\%}$ 	&	 $774^{+1.4\%+2.9\%}_{-1.8\%-2.9\%}$ 	&	 $782.3^{+1.4\%+3.0\%}_{-1.8\%-3.0\%}$ 	\\
	 $100$ 	&	 $160$ 	&	 $130$ 	&	 $1003^{+1.4\%+3.3\%}_{-1.8\%-3.3\%}$ 	&	 $594.8^{+1.5\%+3.3\%}_{-1.9\%-3.3\%}$ 	&	 $1315^{+1.6\%+2.7\%}_{-2.1\%-2.7\%}$ 	&	 $1300^{+1.7\%+2.9\%}_{-2.2\%-2.9\%}$ 	\\
	 $150$ 	&	 $170$ 	&	 $160$ 	&	 $640.7^{+1.2\%+3.5\%}_{-1.5\%-3.5\%}$ 	&	 $369.6^{+1.4\%+3.4\%}_{-1.6\%-3.4\%}$ 	&	 $629.9^{+1.3\%+2.9\%}_{-1.7\%-2.9\%}$ 	&	 $629.2^{+1.4\%+3.1\%}_{-1.7\%-3.1\%}$ 	\\
	 $125$ 	&	 $185$ 	&	 $155$ 	&	 $573.1^{+1.2\%+3.5\%}_{-1.5\%-3.5\%}$ 	&	 $328.4^{+1.3\%+3.5\%}_{-1.6\%-3.5\%}$ 	&	 $705.3^{+1.4\%+2.9\%}_{-1.7\%-2.9\%}$ 	&	 $687.1^{+1.4\%+3.1\%}_{-1.7\%-3.1\%}$ 	\\
	 $175$ 	&	 $195$ 	&	 $185$ 	&	 $388.1^{+1.0\%+3.7\%}_{-1.3\%-3.7\%}$ 	&	 $216.7^{+1.2\%+3.7\%}_{-1.4\%-3.7\%}$ 	&	 $373.8^{+1.1\%+3.1\%}_{-1.4\%-3.1\%}$ 	&	 $367.3^{+1.2\%+3.2\%}_{-1.4\%-3.2\%}$ 	\\
	 $150$ 	&	 $210$ 	&	 $180$ 	&	 $352.1^{+1.0\%+3.7\%}_{-1.2\%-3.7\%}$ 	&	 $195.4^{+1.2\%+3.8\%}_{-1.3\%-3.8\%}$ 	&	 $412.7^{+1.2\%+3.1\%}_{-1.4\%-3.1\%}$ 	&	 $398^{+1.2\%+3.2\%}_{-1.4\%-3.2\%}$ 	\\
	 $200$ 	&	 $230$ 	&	 $215$ 	&	 $219.7^{+0.9\%+3.9\%}_{-1.0\%-3.9\%}$ 	&	 $118^{+1.1\%+4.0\%}_{-1.1\%-4.0\%}$ 	&	 $215.8^{+1.0\%+3.3\%}_{-1.2\%-3.3\%}$ 	&	 $208.6^{+1.0\%+3.5\%}_{-1.2\%-3.5\%}$ 	\\
	 $225$ 	&	 $240$ 	&	 $232.5$ 	&	 $176.7^{+0.8\%+4.1\%}_{-0.9\%-4.1\%}$ 	&	 $93.43^{+1.0\%+4.2\%}_{-1.1\%-4.2\%}$ 	&	 $161.4^{+0.9\%+3.5\%}_{-1.0\%-3.5\%}$ 	&	 $155.5^{+0.9\%+3.6\%}_{-1.1\%-3.6\%}$ 	\\
	 $200$ 	&	 $260$ 	&	 $230$ 	&	 $154.2^{+0.8\%+4.1\%}_{-0.9\%-4.1\%}$ 	&	 $80.73^{+1.0\%+4.3\%}_{-1.0\%-4.3\%}$ 	&	 $168^{+0.9\%+3.4\%}_{-1.1\%-3.4\%}$ 	&	 $159.8^{+0.9\%+3.6\%}_{-1.1\%-3.6\%}$ 	\\
	 $250$ 	&	 $280$ 	&	 $265$ 	&	 $104.3^{+0.7\%+4.4\%}_{-0.8\%-4.4\%}$ 	&	 $53.02^{+0.9\%+4.6\%}_{-0.9\%-4.6\%}$ 	&	 $98.49^{+0.8\%+3.7\%}_{-0.9\%-3.7\%}$ 	&	 $93.86^{+0.8\%+3.8\%}_{-0.9\%-3.8\%}$ 	\\
	 $300$ 	&	 $305$ 	&	 $302.5$ 	&	 $69.32^{+0.6\%+4.7\%}_{-0.7\%-4.7\%}$ 	&	 $34.15^{+0.8\%+5.0\%}_{-0.8\%-5.0\%}$ 	&	 $59.07^{+0.7\%+4.0\%}_{-0.7\%-4.0\%}$ 	&	 $55.98^{+0.7\%+4.1\%}_{-0.7\%-4.1\%}$ 	\\
	 $300$ 	&	 $320$ 	&	 $310$ 	&	 $60.33^{+0.6\%+4.7\%}_{-0.6\%-4.7\%}$ 	&	 $29.39^{+0.7\%+5.1\%}_{-0.7\%-5.1\%}$ 	&	 $53.66^{+0.7\%+4.0\%}_{-0.7\%-4.0\%}$ 	&	 $50.74^{+0.7\%+4.1\%}_{-0.7\%-4.1\%}$ 	\\


==> tab_hinos13000.tex <==
$100$ 	&$3600^{+2.0\%+3.0\%}_{-2.8\%-3.0\%}$ 	&$2275^{+2.1\%+2.9\%}_{-2.9\%-2.9\%}$ 	&$3138^{+2.1\%+2.6\%}_{-2.9\%-2.6\%}$ 	&$3459^{+2.1\%+2.8\%}_{-2.9\%-2.8\%}$ 	\\
	 $200$ 	&	 $303.9^{+0.9\%+3.8\%}_{-1.1\%-3.8\%}$ 	&	 $165.8^{+1.1\%+3.9\%}_{-1.3\%-3.9\%}$ 	&	 $262.9^{+1.0\%+3.3\%}_{-1.2\%-3.3\%}$ 	&	 $256.7^{+1.1\%+3.5\%}_{-1.2\%-3.5\%}$ 	\\
	 $300$ 	&	 $67.64^{+0.6\%+4.7\%}_{-0.6\%-4.7\%}$ 	&	 $33^{+0.8\%+5.1\%}_{-0.8\%-5.1\%}$ 	&	 $56.34^{+0.7\%+4.1\%}_{-0.7\%-4.1\%}$ 	&	 $53.38^{+0.7\%+4.2\%}_{-0.7\%-4.2\%}$ 	\\
	 $400$ 	&	 $21.74^{+0.5\%+5.6\%}_{-0.4\%-5.6\%}$ 	&	 $9.674^{+0.6\%+6.4\%}_{-0.6\%-6.4\%}$ 	&	 $17.46^{+0.5\%+4.9\%}_{-0.5\%-4.9\%}$ 	&	 $16.3^{+0.5\%+5.0\%}_{-0.5\%-5.0\%}$ 	\\
	 $500$ 	&	 $8.496^{+0.5\%+6.5\%}_{-0.3\%-6.5\%}$ 	&	 $3.497^{+0.4\%+7.8\%}_{-0.4\%-7.8\%}$ 	&	 $6.608^{+0.4\%+5.8\%}_{-0.4\%-5.8\%}$ 	&	 $6.108^{+0.4\%+5.9\%}_{-0.4\%-5.9\%}$ 	\\
	 $600$ 	&	 $3.746^{+0.4\%+7.5\%}_{-0.2\%-7.5\%}$ 	&	 $1.442^{+0.4\%+9.4\%}_{-0.3\%-9.4\%}$ 	&	 $2.834^{+0.4\%+6.9\%}_{-0.3\%-6.9\%}$ 	&	 $2.599^{+0.4\%+6.9\%}_{-0.3\%-6.9\%}$ 	\\
	 $700$ 	&	 $1.79^{+0.4\%+8.6\%}_{-0.2\%-8.6\%}$ 	&	 $0.6504^{+0.3\%+11.5\%}_{-0.2\%-11.5\%}$ 	&	 $1.323^{+0.3\%+8.1\%}_{-0.2\%-8.1\%}$ 	&	 $1.206^{+0.4\%+8.1\%}_{-0.2\%-8.1\%}$ 	\\
	 $800$ 	&	 $0.9064^{+0.4\%+10.0\%}_{-0.2\%-10.0\%}$ 	&	 $0.3135^{+0.3\%+14.0\%}_{-0.2\%-14.0\%}$ 	&	 $0.6575^{+0.3\%+9.7\%}_{-0.2\%-9.7\%}$ 	&	 $0.5952^{+0.4\%+9.6\%}_{-0.2\%-9.6\%}$ 	\\
	 $900$ 	&	 $0.4788^{+0.4\%+11.7\%}_{-0.2\%-11.7\%}$ 	&	 $0.1589^{+0.3\%+17.3\%}_{-0.2\%-17.3\%}$ 	&	 $0.3423^{+0.3\%+11.6\%}_{-0.2\%-11.6\%}$ 	&	 $0.3081^{+0.3\%+11.4\%}_{-0.2\%-11.4\%}$ 	\\
	 $1000$ 	&	 $0.2611^{+0.3\%+13.9\%}_{-0.2\%-13.9\%}$ 	&	 $0.08376^{+0.3\%+21.4\%}_{-0.1\%-21.4\%}$ 	&	 $0.1848^{+0.3\%+14.2\%}_{-0.2\%-14.2\%}$ 	&	 $0.1653^{+0.3\%+13.8\%}_{-0.1\%-13.8\%}$ 	\\
	 $1100$ 	&	 $0.146^{+0.3\%+16.9\%}_{-0.1\%-16.9\%}$ 	&	 $0.04559^{+0.3\%+26.5\%}_{-0.1\%-26.5\%}$ 	&	 $0.1028^{+0.3\%+17.4\%}_{-0.1\%-17.4\%}$ 	&	 $0.09133^{+0.3\%+16.8\%}_{-0.1\%-16.8\%}$ 	\\
	 $1200$ 	&	 $0.08327^{+0.3\%+20.9\%}_{-0.1\%-20.9\%}$ 	&	 $0.02548^{+0.2\%+32.8\%}_{-0.1\%-32.8\%}$ 	&	 $0.05856^{+0.3\%+21.5\%}_{-0.1\%-21.5\%}$ 	&	 $0.05169^{+0.3\%+20.7\%}_{-0.1\%-20.7\%}$ 	\\
	 $1300$ 	&	 $0.04826^{+0.3\%+26.2\%}_{-0.1\%-26.2\%}$ 	&	 $0.01457^{+0.2\%+40.6\%}_{-0.1\%-40.6\%}$ 	&	 $0.03405^{+0.2\%+26.6\%}_{-0.1\%-26.6\%}$ 	&	 $0.02986^{+0.3\%+25.6\%}_{-0.1\%-25.6\%}$ 	\\
	 $1400$ 	&	 $0.02837^{+0.3\%+33.1\%}_{-0.1\%-33.1\%}$ 	&	 $0.008485^{+0.2\%+49.9\%}_{-0.1\%-49.9\%}$ 	&	 $0.02015^{+0.3\%+32.8\%}_{-0.1\%-32.8\%}$ 	&	 $0.01755^{+0.3\%+31.6\%}_{-0.1\%-31.6\%}$ 	\\
	 $1500$ 	&	 $0.01687^{+0.3\%+42.0\%}_{-0.1\%-42.0\%}$ 	&	 $0.005026^{+0.2\%+61.0\%}_{-0.1\%-61.0\%}$ 	&	 $0.01211^{+0.2\%+40.5\%}_{-0.1\%-40.5\%}$ 	&	 $0.01048^{+0.2\%+39.0\%}_{-0.1\%-39.0\%}$ 	\\


==> tab_hinos13600.tex <==
$100$ 	&$3806^{+2.1\%+2.9\%}_{-2.9\%-2.9\%}$ 	&$2424^{+2.2\%+2.8\%}_{-3.0\%-2.8\%}$ 	&$3329^{+2.1\%+2.5\%}_{-3.0\%-2.5\%}$ 	&$3673^{+2.2\%+2.7\%}_{-3.0\%-2.7\%}$ 	\\
	 $200$ 	&	 $324.8^{+1.0\%+3.8\%}_{-1.2\%-3.8\%}$ 	&	 $179.2^{+1.2\%+3.8\%}_{-1.3\%-3.8\%}$ 	&	 $282.3^{+1.1\%+3.2\%}_{-1.3\%-3.2\%}$ 	&	 $276.1^{+1.1\%+3.4\%}_{-1.3\%-3.4\%}$ 	\\
	 $300$ 	&	 $73.05^{+0.6\%+4.6\%}_{-0.7\%-4.6\%}$ 	&	 $36.12^{+0.8\%+4.9\%}_{-0.8\%-4.9\%}$ 	&	 $61.2^{+0.7\%+3.9\%}_{-0.7\%-3.9\%}$ 	&	 $58.07^{+0.7\%+4.1\%}_{-0.7\%-4.1\%}$ 	\\
	 $400$ 	&	 $23.74^{+0.5\%+5.5\%}_{-0.4\%-5.5\%}$ 	&	 $10.72^{+0.6\%+6.1\%}_{-0.6\%-6.1\%}$ 	&	 $19.2^{+0.5\%+4.7\%}_{-0.5\%-4.7\%}$ 	&	 $17.94^{+0.5\%+4.9\%}_{-0.5\%-4.9\%}$ 	\\
	 $500$ 	&	 $9.386^{+0.5\%+6.3\%}_{-0.3\%-6.3\%}$ 	&	 $3.926^{+0.5\%+7.4\%}_{-0.5\%-7.4\%}$ 	&	 $7.353^{+0.4\%+5.6\%}_{-0.4\%-5.6\%}$ 	&	 $6.805^{+0.4\%+5.7\%}_{-0.4\%-5.7\%}$ 	\\
	 $600$ 	&	 $4.189^{+0.4\%+7.2\%}_{-0.3\%-7.2\%}$ 	&	 $1.639^{+0.4\%+9.0\%}_{-0.4\%-9.0\%}$ 	&	 $3.192^{+0.4\%+6.6\%}_{-0.3\%-6.6\%}$ 	&	 $2.932^{+0.4\%+6.7\%}_{-0.3\%-6.7\%}$ 	\\
	 $700$ 	&	 $2.028^{+0.4\%+8.2\%}_{-0.2\%-8.2\%}$ 	&	 $0.7493^{+0.3\%+10.8\%}_{-0.3\%-10.8\%}$ 	&	 $1.509^{+0.4\%+7.7\%}_{-0.2\%-7.7\%}$ 	&	 $1.378^{+0.4\%+7.7\%}_{-0.2\%-7.7\%}$ 	\\
	 $800$ 	&	 $1.041^{+0.4\%+9.5\%}_{-0.2\%-9.5\%}$ 	&	 $0.3658^{+0.3\%+13.1\%}_{-0.2\%-13.1\%}$ 	&	 $0.7595^{+0.3\%+9.1\%}_{-0.2\%-9.1\%}$ 	&	 $0.6891^{+0.4\%+9.0\%}_{-0.2\%-9.0\%}$ 	\\
	 $900$ 	&	 $0.5575^{+0.4\%+11.0\%}_{-0.2\%-11.0\%}$ 	&	 $0.1879^{+0.3\%+15.9\%}_{-0.2\%-15.9\%}$ 	&	 $0.4007^{+0.3\%+10.8\%}_{-0.2\%-10.8\%}$ 	&	 $0.3613^{+0.3\%+10.6\%}_{-0.2\%-10.6\%}$ 	\\
	 $1000$ 	&	 $0.3085^{+0.4\%+12.9\%}_{-0.2\%-12.9\%}$ 	&	 $0.1004^{+0.3\%+19.5\%}_{-0.2\%-19.5\%}$ 	&	 $0.2193^{+0.3\%+13.0\%}_{-0.1\%-13.0\%}$ 	&	 $0.1966^{+0.3\%+12.7\%}_{-0.1\%-12.7\%}$ 	\\
	 $1100$ 	&	 $0.1751^{+0.3\%+15.4\%}_{-0.2\%-15.4\%}$ 	&	 $0.05535^{+0.2\%+24.0\%}_{-0.1\%-24.0\%}$ 	&	 $0.1236^{+0.3\%+15.8\%}_{-0.1\%-15.8\%}$ 	&	 $0.1101^{+0.3\%+15.3\%}_{-0.1\%-15.3\%}$ 	\\
	 $1200$ 	&	 $0.1014^{+0.3\%+18.7\%}_{-0.1\%-18.7\%}$ 	&	 $0.03135^{+0.2\%+29.4\%}_{-0.1\%-29.4\%}$ 	&	 $0.07133^{+0.3\%+19.2\%}_{-0.1\%-19.2\%}$ 	&	 $0.06318^{+0.3\%+18.5\%}_{-0.1\%-18.5\%}$ 	\\
	 $1300$ 	&	 $0.0597^{+0.4\%+23.1\%}_{-0.1\%-23.1\%}$ 	&	 $0.01815^{+0.2\%+36.0\%}_{-0.1\%-36.0\%}$ 	&	 $0.04203^{+0.3\%+23.6\%}_{-0.1\%-23.6\%}$ 	&	 $0.03699^{+0.3\%+22.7\%}_{-0.1\%-22.7\%}$ 	\\
	 $1400$ 	&	 $0.03564^{+0.3\%+28.7\%}_{-0.1\%-28.7\%}$ 	&	 $0.01071^{+0.2\%+44.0\%}_{-0.2\%-44.0\%}$ 	&	 $0.02521^{+0.3\%+28.9\%}_{-0.1\%-28.9\%}$ 	&	 $0.02204^{+0.3\%+27.8\%}_{-0.1\%-27.8\%}$ 	\\
	 $1500$ 	&	 $0.02153^{+0.3\%+35.9\%}_{-0.1\%-35.9\%}$ 	&	 $0.006428^{+0.2\%+53.5\%}_{-0.1\%-53.5\%}$ 	&	 $0.01535^{+0.3\%+35.4\%}_{-0.1\%-35.4\%}$ 	&	 $0.01333^{+0.2\%+34.1\%}_{-0.1\%-34.1\%}$ 	\\


==> tab_sleptons13000.tex <==
$100$ 	&$282.2^{+1.6\%+2.7\%}_{-2.3\%-2.7\%}$ 	&$100.6^{+1.6\%+3.0\%}_{-2.3\%-3.0\%}$ 	&$116.7^{+1.6\%+3.1\%}_{-2.3\%-3.1\%}$ 	\\
	 $200$ 	&	 $22.71^{+1.0\%+3.5\%}_{-0.8\%-3.5\%}$ 	&	 $8.484^{+1.1\%+3.7\%}_{-0.8\%-3.7\%}$ 	&	 $10.13^{+1.1\%+3.8\%}_{-0.8\%-3.8\%}$ 	\\
	 $300$ 	&	 $4.62^{+0.7\%+4.5\%}_{-0.5\%-4.5\%}$ 	&	 $1.753^{+0.7\%+4.6\%}_{-0.5\%-4.6\%}$ 	&	 $2.101^{+0.7\%+4.6\%}_{-0.5\%-4.6\%}$ 	\\
	 $400$ 	&	 $1.361^{+0.6\%+5.5\%}_{-0.4\%-5.5\%}$ 	&	 $0.5209^{+0.6\%+5.7\%}_{-0.4\%-5.7\%}$ 	&	 $0.6254^{+0.6\%+5.7\%}_{-0.4\%-5.7\%}$ 	\\
	 $500$ 	&	 $0.4901^{+0.5\%+6.7\%}_{-0.3\%-6.7\%}$ 	&	 $0.1888^{+0.5\%+6.9\%}_{-0.3\%-6.9\%}$ 	&	 $0.2269^{+0.5\%+6.9\%}_{-0.3\%-6.9\%}$ 	\\
	 $600$ 	&	 $0.2004^{+0.4\%+8.1\%}_{-0.2\%-8.1\%}$ 	&	 $0.07765^{+0.4\%+8.4\%}_{-0.2\%-8.4\%}$ 	&	 $0.09334^{+0.4\%+8.4\%}_{-0.2\%-8.4\%}$ 	\\
	 $700$ 	&	 $0.0894^{+0.4\%+9.9\%}_{-0.2\%-9.9\%}$ 	&	 $0.03482^{+0.4\%+10.3\%}_{-0.2\%-10.3\%}$ 	&	 $0.04188^{+0.4\%+10.4\%}_{-0.2\%-10.4\%}$ 	\\
	 $800$ 	&	 $0.0425^{+0.4\%+12.3\%}_{-0.2\%-12.3\%}$ 	&	 $0.01664^{+0.4\%+12.9\%}_{-0.2\%-12.9\%}$ 	&	 $0.02002^{+0.4\%+12.9\%}_{-0.2\%-12.9\%}$ 	\\
	 $900$ 	&	 $0.02121^{+0.5\%+15.4\%}_{-0.2\%-15.4\%}$ 	&	 $0.008347^{+0.5\%+16.2\%}_{-0.2\%-16.2\%}$ 	&	 $0.01004^{+0.5\%+16.2\%}_{-0.2\%-16.2\%}$ 	\\
	 $1000$ 	&	 $0.01101^{+0.4\%+19.3\%}_{-0.1\%-19.3\%}$ 	&	 $0.004354^{+0.4\%+20.4\%}_{-0.1\%-20.4\%}$ 	&	 $0.00524^{+0.4\%+20.4\%}_{-0.1\%-20.4\%}$ 	\\


==> tab_sleptons13600.tex <==
$100$ 	&$300.2^{+1.7\%+2.7\%}_{-2.4\%-2.7\%}$ 	&$106.9^{+1.7\%+3.0\%}_{-2.4\%-3.0\%}$ 	&$124^{+1.7\%+3.1\%}_{-2.4\%-3.1\%}$ 	\\
	 $200$ 	&	 $24.51^{+1.1\%+3.5\%}_{-0.9\%-3.5\%}$ 	&	 $9.145^{+1.1\%+3.7\%}_{-0.9\%-3.7\%}$ 	&	 $10.92^{+1.1\%+3.7\%}_{-0.9\%-3.7\%}$ 	\\
	 $300$ 	&	 $5.053^{+0.7\%+4.4\%}_{-0.5\%-4.4\%}$ 	&	 $1.915^{+0.8\%+4.5\%}_{-0.5\%-4.5\%}$ 	&	 $2.296^{+0.8\%+4.5\%}_{-0.5\%-4.5\%}$ 	\\
	 $400$ 	&	 $1.509^{+0.6\%+5.4\%}_{-0.4\%-5.4\%}$ 	&	 $0.5768^{+0.6\%+5.5\%}_{-0.4\%-5.5\%}$ 	&	 $0.6925^{+0.6\%+5.5\%}_{-0.4\%-5.5\%}$ 	\\
	 $500$ 	&	 $0.551^{+0.5\%+6.4\%}_{-0.3\%-6.4\%}$ 	&	 $0.2121^{+0.5\%+6.6\%}_{-0.3\%-6.6\%}$ 	&	 $0.2548^{+0.5\%+6.6\%}_{-0.3\%-6.6\%}$ 	\\
	 $600$ 	&	 $0.2285^{+0.4\%+7.7\%}_{-0.3\%-7.7\%}$ 	&	 $0.08842^{+0.4\%+7.9\%}_{-0.3\%-7.9\%}$ 	&	 $0.1063^{+0.5\%+8.0\%}_{-0.3\%-8.0\%}$ 	\\
	 $700$ 	&	 $0.1034^{+0.4\%+9.3\%}_{-0.2\%-9.3\%}$ 	&	 $0.04021^{+0.4\%+9.7\%}_{-0.2\%-9.7\%}$ 	&	 $0.04835^{+0.4\%+9.7\%}_{-0.2\%-9.7\%}$ 	\\
	 $800$ 	&	 $0.04985^{+0.4\%+11.4\%}_{-0.2\%-11.4\%}$ 	&	 $0.01949^{+0.4\%+11.9\%}_{-0.2\%-11.9\%}$ 	&	 $0.02344^{+0.4\%+11.9\%}_{-0.2\%-11.9\%}$ 	\\
	 $900$ 	&	 $0.02523^{+0.4\%+14.1\%}_{-0.2\%-14.1\%}$ 	&	 $0.009911^{+0.5\%+14.8\%}_{-0.2\%-14.8\%}$ 	&	 $0.01192^{+0.5\%+14.9\%}_{-0.2\%-14.9\%}$ 	\\
	 $1000$ 	&	 $0.01328^{+0.4\%+17.5\%}_{-0.1\%-17.5\%}$ 	&	 $0.005242^{+0.4\%+18.5\%}_{-0.1\%-18.5\%}$ 	&	 $0.006309^{+0.4\%+18.5\%}_{-0.1\%-18.5\%}$ 	\\


==> tab_winos13000.tex <==
$100$ 	&$14400^{+2.0\%+3.0\%}_{-2.8\%-3.0\%}$ 	&$9101^{+2.1\%+2.9\%}_{-2.9\%-2.9\%}$ 	&$12090^{+2.1\%+2.6\%}_{-2.9\%-2.6\%}$ 	\\
	 $200$ 	&	 $1216^{+0.9\%+3.8\%}_{-1.1\%-3.8\%}$ 	&	 $663.2^{+1.1\%+3.9\%}_{-1.3\%-3.9\%}$ 	&	 $941.9^{+1.0\%+3.3\%}_{-1.2\%-3.3\%}$ 	\\
	 $300$ 	&	 $270.5^{+0.6\%+4.7\%}_{-0.6\%-4.7\%}$ 	&	 $132^{+0.8\%+5.1\%}_{-0.8\%-5.1\%}$ 	&	 $198.2^{+0.7\%+4.1\%}_{-0.7\%-4.1\%}$ 	\\
	 $400$ 	&	 $86.95^{+0.5\%+5.6\%}_{-0.4\%-5.6\%}$ 	&	 $38.69^{+0.6\%+6.4\%}_{-0.6\%-6.4\%}$ 	&	 $60.87^{+0.5\%+4.9\%}_{-0.5\%-4.9\%}$ 	\\
	 $500$ 	&	 $33.98^{+0.5\%+6.5\%}_{-0.3\%-6.5\%}$ 	&	 $13.99^{+0.4\%+7.8\%}_{-0.4\%-7.8\%}$ 	&	 $22.89^{+0.4\%+5.8\%}_{-0.4\%-5.8\%}$ 	\\
	 $600$ 	&	 $14.98^{+0.4\%+7.5\%}_{-0.2\%-7.5\%}$ 	&	 $5.765^{+0.4\%+9.4\%}_{-0.3\%-9.4\%}$ 	&	 $9.769^{+0.4\%+6.9\%}_{-0.3\%-6.9\%}$ 	\\
	 $700$ 	&	 $7.159^{+0.4\%+8.6\%}_{-0.2\%-8.6\%}$ 	&	 $2.601^{+0.3\%+11.5\%}_{-0.2\%-11.5\%}$ 	&	 $4.543^{+0.3\%+8.1\%}_{-0.2\%-8.1\%}$ 	\\
	 $800$ 	&	 $3.624^{+0.4\%+10.0\%}_{-0.2\%-10.0\%}$ 	&	 $1.253^{+0.3\%+14.0\%}_{-0.2\%-14.0\%}$ 	&	 $2.248^{+0.4\%+9.5\%}_{-0.2\%-9.5\%}$ 	\\
	 $900$ 	&	 $1.914^{+0.4\%+11.7\%}_{-0.2\%-11.7\%}$ 	&	 $0.6351^{+0.3\%+17.3\%}_{-0.2\%-17.3\%}$ 	&	 $1.166^{+0.3\%+11.4\%}_{-0.2\%-11.4\%}$ 	\\
	 $1000$ 	&	 $1.044^{+0.3\%+13.9\%}_{-0.2\%-13.9\%}$ 	&	 $0.3348^{+0.3\%+21.4\%}_{-0.1\%-21.4\%}$ 	&	 $0.6272^{+0.3\%+13.8\%}_{-0.1\%-13.8\%}$ 	\\
	 $1100$ 	&	 $0.5836^{+0.3\%+16.9\%}_{-0.1\%-16.9\%}$ 	&	 $0.1822^{+0.3\%+26.5\%}_{-0.1\%-26.5\%}$ 	&	 $0.3474^{+0.3\%+16.9\%}_{-0.1\%-16.9\%}$ 	\\
	 $1200$ 	&	 $0.3328^{+0.3\%+20.9\%}_{-0.1\%-20.9\%}$ 	&	 $0.1018^{+0.2\%+32.8\%}_{-0.1\%-32.8\%}$ 	&	 $0.1971^{+0.3\%+20.9\%}_{-0.1\%-20.9\%}$ 	\\
	 $1300$ 	&	 $0.1929^{+0.3\%+26.2\%}_{-0.1\%-26.2\%}$ 	&	 $0.0582^{+0.2\%+40.6\%}_{-0.1\%-40.6\%}$ 	&	 $0.1141^{+0.3\%+25.8\%}_{-0.1\%-25.8\%}$ 	\\
	 $1400$ 	&	 $0.1133^{+0.3\%+33.0\%}_{-0.1\%-33.0\%}$ 	&	 $0.0339^{+0.2\%+49.8\%}_{-0.1\%-49.8\%}$ 	&	 $0.06724^{+0.3\%+31.9\%}_{-0.1\%-31.9\%}$ 	\\
	 $1500$ 	&	 $0.06738^{+0.3\%+42.0\%}_{-0.1\%-42.0\%}$ 	&	 $0.02008^{+0.2\%+61.0\%}_{-0.1\%-61.0\%}$ 	&	 $0.04025^{+0.2\%+39.4\%}_{-0.1\%-39.4\%}$ 	\\
	 $1600$ 	&	 $0.0405^{+0.3\%+53.5\%}_{-0.1\%-53.5\%}$ 	&	 $0.01207^{+0.2\%+74.0\%}_{-0.1\%-74.0\%}$ 	&	 $0.02442^{+0.2\%+48.5\%}_{-0.1\%-48.5\%}$ 	\\
	 $1700$ 	&	 $0.02458^{+0.2\%+68.0\%}_{-0.1\%-68.0\%}$ 	&	 $0.00735^{+0.2\%+89.3\%}_{-0.1\%-89.3\%}$ 	&	 $0.01501^{+0.2\%+59.3\%}_{-0.1\%-59.3\%}$ 	\\
	 $1800$ 	&	 $0.01507^{+0.2\%+86.2\%}_{-0.0\%-86.2\%}$ 	&	 $0.004532^{+0.2\%+107.0\%}_{-0.0\%-107.0\%}$ 	&	 $0.009333^{+0.2\%+72.2\%}_{-0.0\%-72.2\%}$ 	\\
	 $1900$ 	&	 $0.00933^{+0.2\%+108.5\%}_{-0.0\%-108.5\%}$ 	&	 $0.002825^{+0.2\%+127.0\%}_{-0.0\%-127.0\%}$ 	&	 $0.005867^{+0.2\%+87.2\%}_{-0.0\%-87.2\%}$ 	\\
	 $2000$ 	&	 $0.005834^{+0.2\%+135.7\%}_{-0.0\%-135.7\%}$ 	&	 $0.001778^{+0.2\%+149.6\%}_{-0.0\%-149.6\%}$ 	&	 $0.003727^{+0.2\%+104.8\%}_{-0.0\%-104.8\%}$ 	\\


==> tab_winos13600.tex <==
$100$ 	&$15220^{+2.1\%+2.9\%}_{-2.9\%-2.9\%}$ 	&$9695^{+2.2\%+2.8\%}_{-3.0\%-2.8\%}$ 	&$12840^{+2.2\%+2.6\%}_{-3.0\%-2.6\%}$ 	\\
	 $200$ 	&	 $1299^{+1.0\%+3.8\%}_{-1.2\%-3.8\%}$ 	&	 $716.7^{+1.2\%+3.8\%}_{-1.3\%-3.8\%}$ 	&	 $1012^{+1.1\%+3.3\%}_{-1.3\%-3.3\%}$ 	\\
	 $300$ 	&	 $292.2^{+0.6\%+4.6\%}_{-0.7\%-4.6\%}$ 	&	 $144.5^{+0.8\%+4.9\%}_{-0.8\%-4.9\%}$ 	&	 $215.5^{+0.7\%+4.0\%}_{-0.7\%-4.0\%}$ 	\\
	 $400$ 	&	 $94.95^{+0.5\%+5.5\%}_{-0.4\%-5.5\%}$ 	&	 $42.89^{+0.6\%+6.1\%}_{-0.6\%-6.1\%}$ 	&	 $66.96^{+0.5\%+4.8\%}_{-0.5\%-4.8\%}$ 	\\
	 $500$ 	&	 $37.54^{+0.5\%+6.3\%}_{-0.3\%-6.3\%}$ 	&	 $15.7^{+0.5\%+7.4\%}_{-0.5\%-7.4\%}$ 	&	 $25.49^{+0.4\%+5.6\%}_{-0.4\%-5.6\%}$ 	\\
	 $600$ 	&	 $16.75^{+0.4\%+7.2\%}_{-0.3\%-7.2\%}$ 	&	 $6.556^{+0.4\%+9.0\%}_{-0.4\%-9.0\%}$ 	&	 $11.01^{+0.4\%+6.6\%}_{-0.3\%-6.6\%}$ 	\\
	 $700$ 	&	 $8.11^{+0.4\%+8.2\%}_{-0.2\%-8.2\%}$ 	&	 $2.996^{+0.3\%+10.8\%}_{-0.3\%-10.8\%}$ 	&	 $5.188^{+0.4\%+7.7\%}_{-0.2\%-7.7\%}$ 	\\
	 $800$ 	&	 $4.161^{+0.4\%+9.5\%}_{-0.2\%-9.5\%}$ 	&	 $1.463^{+0.3\%+13.1\%}_{-0.2\%-13.1\%}$ 	&	 $2.601^{+0.4\%+9.0\%}_{-0.2\%-9.0\%}$ 	\\
	 $900$ 	&	 $2.229^{+0.4\%+11.0\%}_{-0.2\%-11.0\%}$ 	&	 $0.7511^{+0.3\%+15.9\%}_{-0.2\%-15.9\%}$ 	&	 $1.367^{+0.3\%+10.6\%}_{-0.2\%-10.6\%}$ 	\\
	 $1000$ 	&	 $1.233^{+0.4\%+12.9\%}_{-0.2\%-12.9\%}$ 	&	 $0.4012^{+0.3\%+19.5\%}_{-0.2\%-19.5\%}$ 	&	 $0.7451^{+0.3\%+12.7\%}_{-0.1\%-12.7\%}$ 	\\
	 $1100$ 	&	 $0.6999^{+0.3\%+15.4\%}_{-0.2\%-15.4\%}$ 	&	 $0.2212^{+0.2\%+24.0\%}_{-0.1\%-24.0\%}$ 	&	 $0.4183^{+0.3\%+15.4\%}_{-0.1\%-15.4\%}$ 	\\
	 $1200$ 	&	 $0.4052^{+0.3\%+18.7\%}_{-0.1\%-18.7\%}$ 	&	 $0.1253^{+0.2\%+29.4\%}_{-0.1\%-29.4\%}$ 	&	 $0.2406^{+0.3\%+18.7\%}_{-0.1\%-18.7\%}$ 	\\
	 $1300$ 	&	 $0.2385^{+0.4\%+23.1\%}_{-0.1\%-23.1\%}$ 	&	 $0.07254^{+0.2\%+36.0\%}_{-0.1\%-36.0\%}$ 	&	 $0.1412^{+0.3\%+22.9\%}_{-0.1\%-22.9\%}$ 	\\
	 $1400$ 	&	 $0.1424^{+0.3\%+28.7\%}_{-0.1\%-28.7\%}$ 	&	 $0.0428^{+0.2\%+44.0\%}_{-0.2\%-44.0\%}$ 	&	 $0.08431^{+0.3\%+28.1\%}_{-0.1\%-28.1\%}$ 	\\
	 $1500$ 	&	 $0.08599^{+0.3\%+35.9\%}_{-0.1\%-35.9\%}$ 	&	 $0.02568^{+0.2\%+53.5\%}_{-0.1\%-53.5\%}$ 	&	 $0.05113^{+0.2\%+34.4\%}_{-0.1\%-34.4\%}$ 	\\
	 $1600$ 	&	 $0.05247^{+0.3\%+45.3\%}_{-0.1\%-45.3\%}$ 	&	 $0.01563^{+0.2\%+64.7\%}_{-0.1\%-64.7\%}$ 	&	 $0.03143^{+0.2\%+42.0\%}_{-0.1\%-42.0\%}$ 	\\
	 $1700$ 	&	 $0.03233^{+0.2\%+57.0\%}_{-0.1\%-57.0\%}$ 	&	 $0.00964^{+0.2\%+77.8\%}_{-0.1\%-77.8\%}$ 	&	 $0.01956^{+0.2\%+51.1\%}_{-0.1\%-51.1\%}$ 	\\
	 $1800$ 	&	 $0.0201^{+0.2\%+71.7\%}_{-0.1\%-71.7\%}$ 	&	 $0.006017^{+0.2\%+92.9\%}_{-0.0\%-92.9\%}$ 	&	 $0.01231^{+0.2\%+62.0\%}_{-0.0\%-62.0\%}$ 	\\
	 $1900$ 	&	 $0.01261^{+0.2\%+89.8\%}_{-0.0\%-89.8\%}$ 	&	 $0.003797^{+0.2\%+110.3\%}_{-0.0\%-110.3\%}$ 	&	 $0.007831^{+0.2\%+74.6\%}_{-0.0\%-74.6\%}$ 	\\
	 $2000$ 	&	 $0.007983^{+0.2\%+111.9\%}_{-0.0\%-111.9\%}$ 	&	 $0.002419^{+0.2\%+129.8\%}_{-0.0\%-129.8\%}$ 	&	 $0.005031^{+0.2\%+89.4\%}_{-0.0\%-89.4\%}$ 	\\


==> tab_winosq13000.tex <==
$700$ 	&$700$ 	&$0.2825^{+12.5\%+7.9\%}_{-9.4\%-7.9\%}$ 	&$0.1098^{+14.2\%+13.0\%}_{-10.6\%-13.0\%}$ 	&$1.092^{+6.2\%+9.4\%}_{-4.5\%-9.4\%}$ 	\\
	 $2600$ 	&	 $700$ 	&	 $4.426^{+0.6\%+8.3\%}_{-0.5\%-8.3\%}$ 	&	 $1.623^{+0.8\%+10.8\%}_{-0.6\%-10.8\%}$ 	&	 $2.899^{+0.7\%+7.8\%}_{-0.5\%-7.8\%}$ 	\\
	 $1200$ 	&	 $800$ 	&	 $0.286^{+4.8\%+9.0\%}_{-5.3\%-9.0\%}$ 	&	 $0.1035^{+4.3\%+12.6\%}_{-4.3\%-12.6\%}$ 	&	 $0.4114^{+0.7\%+11.1\%}_{-0.2\%-11.1\%}$ 	\\
	 $3100$ 	&	 $800$ 	&	 $2.355^{+0.4\%+9.5\%}_{-0.4\%-9.5\%}$ 	&	 $0.8206^{+0.7\%+13.2\%}_{-0.5\%-13.2\%}$ 	&	 $1.496^{+0.5\%+9.2\%}_{-0.5\%-9.2\%}$ 	\\
	 $1800$ 	&	 $900$ 	&	 $0.4462^{+2.3\%+10.6\%}_{-2.7\%-10.6\%}$ 	&	 $0.1501^{+2.5\%+15.5\%}_{-2.7\%-15.5\%}$ 	&	 $0.3419^{+1.5\%+11.7\%}_{-1.5\%-11.7\%}$ 	\\
	 $3700$ 	&	 $900$ 	&	 $1.317^{+0.3\%+11.1\%}_{-0.3\%-11.1\%}$ 	&	 $0.439^{+0.5\%+16.3\%}_{-0.4\%-16.3\%}$ 	&	 $0.8152^{+0.4\%+10.9\%}_{-0.4\%-10.9\%}$ 	\\
	 $2500$ 	&	 $1000$ 	&	 $0.4081^{+1.2\%+12.7\%}_{-1.2\%-12.7\%}$ 	&	 $0.1319^{+1.4\%+19.4\%}_{-1.4\%-19.4\%}$ 	&	 $0.2674^{+1.0\%+13.3\%}_{-0.9\%-13.3\%}$ 	\\
	 $1400$ 	&	 $1100$ 	&	 $0.02048^{+3.8\%+15.8\%}_{-4.0\%-15.8\%}$ 	&	 $0.007046^{+1.6\%+24.9\%}_{-1.5\%-24.9\%}$ 	&	 $0.05042^{+1.9\%+23.1\%}_{-1.1\%-23.1\%}$ 	\\
	 $3300$ 	&	 $1100$ 	&	 $0.3041^{+0.6\%+15.4\%}_{-0.6\%-15.4\%}$ 	&	 $0.09535^{+0.8\%+24.3\%}_{-0.7\%-24.3\%}$ 	&	 $0.1882^{+0.6\%+16.0\%}_{-0.6\%-16.0\%}$ 	\\
	 $2300$ 	&	 $1200$ 	&	 $0.07346^{+2.3\%+18.2\%}_{-2.7\%-18.2\%}$ 	&	 $0.0226^{+2.5\%+29.2\%}_{-2.8\%-29.2\%}$ 	&	 $0.05376^{+1.5\%+21.4\%}_{-1.6\%-21.4\%}$ 	\\
	 $1400$ 	&	 $1300$ 	&	 $0.004227^{+12.1\%+32.1\%}_{-8.6\%-32.1\%}$ 	&	 $0.001485^{+14.7\%+41.9\%}_{-10.5\%-41.9\%}$ 	&	 $0.01734^{+5.4\%+36.7\%}_{-3.8\%-36.7\%}$ 	\\
	 $3300$ 	&	 $1300$ 	&	 $0.08107^{+0.9\%+23.1\%}_{-1.0\%-23.1\%}$ 	&	 $0.0245^{+1.1\%+36.8\%}_{-1.1\%-36.8\%}$ 	&	 $0.05094^{+0.9\%+24.5\%}_{-0.9\%-24.5\%}$ 	\\
	 $2500$ 	&	 $1400$ 	&	 $0.02079^{+2.6\%+28.2\%}_{-3.2\%-28.2\%}$ 	&	 $0.006229^{+2.8\%+44.3\%}_{-3.2\%-44.3\%}$ 	&	 $0.01588^{+1.6\%+33.6\%}_{-1.8\%-33.6\%}$ 	\\
	 $1800$ 	&	 $1500$ 	&	 $0.00174^{+1.2\%+42.4\%}_{-1.0\%-42.4\%}$ 	&	 $0.000566^{+2.4\%+54.7\%}_{-1.3\%-54.7\%}$ 	&	 $0.005011^{+2.7\%+56.5\%}_{-1.5\%-56.5\%}$ 	\\
	 $3700$ 	&	 $1500$ 	&	 $0.02763^{+0.9\%+36.9\%}_{-1.1\%-36.9\%}$ 	&	 $0.008222^{+1.1\%+55.7\%}_{-1.1\%-55.7\%}$ 	&	 $0.01746^{+0.9\%+37.4\%}_{-0.9\%-37.4\%}$ 	\\
	 $3100$ 	&	 $1600$ 	&	 $0.009849^{+1.8\%+46.0\%}_{-2.3\%-46.0\%}$ 	&	 $0.002928^{+2.0\%+66.7\%}_{-2.3\%-66.7\%}$ 	&	 $0.006916^{+1.4\%+48.5\%}_{-1.6\%-48.5\%}$ 	\\
	 $2600$ 	&	 $1700$ 	&	 $0.00255^{+3.7\%+58.3\%}_{-4.6\%-58.3\%}$ 	&	 $0.0007621^{+3.7\%+79.5\%}_{-4.4\%-79.5\%}$ 	&	 $0.002462^{+1.6\%+68.3\%}_{-1.9\%-68.3\%}$ 	\\
	 $2200$ 	&	 $1800$ 	&	 $0.0004346^{+2.1\%+79.2\%}_{-2.0\%-79.2\%}$ 	&	 $0.0001349^{+1.2\%+92.2\%}_{-1.0\%-92.2\%}$ 	&	 $0.001059^{+1.6\%+99.8\%}_{-0.9\%-99.8\%}$ 	\\
	 $1900$ 	&	 $1900$ 	&	 $0.0002043^{+17.9\%+136.6\%}_{-13.1\%-136.6\%}$ 	&	 $6.368e-05^{+18.4\%+137.1\%}_{-13.4\%-137.1\%}$ 	&	 $0.0008132^{+6.3\%+121.4\%}_{-4.6\%-121.4\%}$ 	\\
	 $3800$ 	&	 $1900$ 	&	 $0.002555^{+1.6\%+95.2\%}_{-1.9\%-95.2\%}$ 	&	 $0.0007716^{+1.5\%+116.8\%}_{-1.9\%-116.8\%}$ 	&	 $0.001798^{+1.2\%+85.7\%}_{-1.4\%-85.7\%}$ 	\\
	 $3600$ 	&	 $2000$ 	&	 $0.001189^{+2.0\%+118.9\%}_{-2.5\%-118.9\%}$ 	&	 $0.000362^{+2.0\%+137.3\%}_{-2.5\%-137.3\%}$ 	&	 $0.0009069^{+1.4\%+105.6\%}_{-1.6\%-105.6\%}$ 	\\


==> tab_winosq13600.tex <==
$700$ 	&$700$ 	&$0.3311^{+12.3\%+7.4\%}_{-9.3\%-7.4\%}$ 	&$0.1305^{+14.0\%+12.1\%}_{-10.5\%-12.1\%}$ 	&$1.27^{+6.1\%+8.8\%}_{-4.5\%-8.8\%}$ 	\\
	 $2600$ 	&	 $700$ 	&	 $4.996^{+0.6\%+7.9\%}_{-0.5\%-7.9\%}$ 	&	 $1.865^{+0.8\%+10.2\%}_{-0.7\%-10.2\%}$ 	&	 $3.303^{+0.7\%+7.4\%}_{-0.5\%-7.4\%}$ 	\\
	 $1200$ 	&	 $800$ 	&	 $0.3305^{+4.5\%+8.0\%}_{-5.1\%-8.0\%}$ 	&	 $0.1216^{+4.0\%+12.0\%}_{-4.1\%-12.0\%}$ 	&	 $0.4831^{+0.5\%+10.3\%}_{-0.1\%-10.3\%}$ 	\\
	 $3100$ 	&	 $800$ 	&	 $2.695^{+0.5\%+9.1\%}_{-0.4\%-9.1\%}$ 	&	 $0.955^{+0.7\%+12.3\%}_{-0.5\%-12.3\%}$ 	&	 $1.727^{+0.5\%+8.7\%}_{-0.4\%-8.7\%}$ 	\\
	 $1800$ 	&	 $900$ 	&	 $0.5166^{+2.4\%+10.0\%}_{-2.6\%-10.0\%}$ 	&	 $0.1766^{+2.6\%+14.1\%}_{-2.6\%-14.1\%}$ 	&	 $0.4015^{+1.5\%+10.8\%}_{-1.3\%-10.8\%}$ 	\\
	 $3700$ 	&	 $900$ 	&	 $1.528^{+0.3\%+10.5\%}_{-0.3\%-10.5\%}$ 	&	 $0.5178^{+0.5\%+15.0\%}_{-0.5\%-15.0\%}$ 	&	 $0.9535^{+0.4\%+10.2\%}_{-0.4\%-10.2\%}$ 	\\
	 $2500$ 	&	 $1000$ 	&	 $0.4795^{+1.2\%+11.8\%}_{-1.2\%-11.8\%}$ 	&	 $0.1573^{+1.4\%+17.7\%}_{-1.4\%-17.7\%}$ 	&	 $0.3171^{+1.0\%+12.3\%}_{-0.9\%-12.3\%}$ 	\\
	 $1400$ 	&	 $1100$ 	&	 $0.02503^{+3.4\%+14.3\%}_{-3.2\%-14.3\%}$ 	&	 $0.008748^{+1.1\%+22.8\%}_{-1.6\%-22.8\%}$ 	&	 $0.06213^{+2.0\%+20.8\%}_{-1.1\%-20.8\%}$ 	\\
	 $3300$ 	&	 $1100$ 	&	 $0.363^{+0.6\%+14.1\%}_{-0.6\%-14.1\%}$ 	&	 $0.1153^{+0.9\%+21.9\%}_{-0.7\%-21.9\%}$ 	&	 $0.226^{+0.6\%+14.6\%}_{-0.6\%-14.6\%}$ 	\\
	 $2300$ 	&	 $1200$ 	&	 $0.08891^{+2.2\%+16.3\%}_{-2.6\%-16.3\%}$ 	&	 $0.02766^{+2.4\%+26.1\%}_{-2.6\%-26.1\%}$ 	&	 $0.0657^{+1.5\%+19.2\%}_{-1.6\%-19.2\%}$ 	\\
	 $1400$ 	&	 $1300$ 	&	 $0.005441^{+12.0\%+28.0\%}_{-8.6\%-28.0\%}$ 	&	 $0.001926^{+14.5\%+37.7\%}_{-10.4\%-37.7\%}$ 	&	 $0.02201^{+5.4\%+32.4\%}_{-3.8\%-32.4\%}$ 	\\
	 $3300$ 	&	 $1300$ 	&	 $0.09974^{+0.9\%+20.4\%}_{-1.0\%-20.4\%}$ 	&	 $0.03039^{+1.1\%+32.6\%}_{-1.1\%-32.6\%}$ 	&	 $0.06287^{+0.9\%+21.8\%}_{-0.8\%-21.8\%}$ 	\\
	 $2500$ 	&	 $1400$ 	&	 $0.02597^{+2.5\%+24.6\%}_{-3.1\%-24.6\%}$ 	&	 $0.007827^{+2.8\%+39.0\%}_{-3.0\%-39.0\%}$ 	&	 $0.01995^{+1.6\%+29.6\%}_{-1.6\%-29.6\%}$ 	\\
	 $1800$ 	&	 $1500$ 	&	 $0.00227^{+1.0\%+36.7\%}_{-0.8\%-36.7\%}$ 	&	 $0.0007457^{+2.7\%+48.7\%}_{-1.7\%-48.7\%}$ 	&	 $0.006532^{+2.7\%+49.3\%}_{-1.6\%-49.3\%}$ 	\\
	 $3700$ 	&	 $1500$ 	&	 $0.03507^{+0.9\%+31.6\%}_{-1.0\%-31.6\%}$ 	&	 $0.01047^{+1.0\%+48.7\%}_{-1.1\%-48.7\%}$ 	&	 $0.02214^{+0.8\%+32.7\%}_{-0.8\%-32.7\%}$ 	\\
	 $3100$ 	&	 $1600$ 	&	 $0.01269^{+1.8\%+39.0\%}_{-2.3\%-39.0\%}$ 	&	 $0.003775^{+2.0\%+58.2\%}_{-2.3\%-58.2\%}$ 	&	 $0.0089^{+1.3\%+42.1\%}_{-1.5\%-42.1\%}$ 	\\
	 $2600$ 	&	 $1700$ 	&	 $0.003341^{+3.5\%+49.0\%}_{-4.4\%-49.0\%}$ 	&	 $0.0009981^{+3.5\%+69.2\%}_{-4.2\%-69.2\%}$ 	&	 $0.003236^{+1.6\%+59.3\%}_{-1.7\%-59.3\%}$ 	\\
	 $2200$ 	&	 $1800$ 	&	 $0.0005891^{+1.8\%+66.8\%}_{-1.8\%-66.8\%}$ 	&	 $0.0001838^{+0.8\%+81.5\%}_{-0.8\%-81.5\%}$ 	&	 $0.001432^{+1.7\%+86.3\%}_{-1.1\%-86.3\%}$ 	\\
	 $1900$ 	&	 $1900$ 	&	 $0.0002842^{+17.6\%+115.0\%}_{-12.9\%-115.0\%}$ 	&	 $8.894e-05^{+18.1\%+120.2\%}_{-13.3\%-120.2\%}$ 	&	 $0.001113^{+6.2\%+104.7\%}_{-4.5\%-104.7\%}$ 	\\
	 $3800$ 	&	 $1900$ 	&	 $0.003438^{+1.5\%+78.4\%}_{-1.8\%-78.4\%}$ 	&	 $0.001032^{+1.6\%+100.9\%}_{-1.8\%-100.9\%}$ 	&	 $0.002398^{+1.2\%+73.5\%}_{-1.3\%-73.5\%}$ 	\\
	 $3600$ 	&	 $2000$ 	&	 $0.001621^{+2.1\%+97.4\%}_{-2.5\%-97.4\%}$ 	&	 $0.0004901^{+2.0\%+118.5\%}_{-2.5\%-118.5\%}$ 	&	 $0.001226^{+1.4\%+90.7\%}_{-1.6\%-90.7\%}$ 	\\

